Celer: an Efficient Program for Genotype Elimination

This paper presents an efficient program for checking Mendelian consistency in a pedigree. Since pedigrees may contain incomplete and/or erroneous information, geneticists need to pre-process them before performing linkage analysis. Removing superfluous genotypes that do not respect the Mendelian inheritance laws can speed up the linkage analysis. We have described in a formal way the Mendelian consistency problem and algorithms known in literature. The formalization helped to polish the algorithms and to find efficient data structures. The performance of the tool has been tested on a wide range of benchmarks. The results are promising if compared to other programs that treat Mendelian consistency.

==> eptcsdata.tex <==
\providecommand{\firstpage}{56}
\providecommand{\publicationstatus}{P. Milazzo and M.J. P\'erez Jim\'enez (Eds.): Applications of Membrane Computing,\\
Concurrency and Agent-based Modelling in Population Biology (AMCA-POP 2010)\\
EPTCS 33, 2010, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.33.4}{10.4204/EPTCS.33.4}}

